Niyama : Breaking the Silos of LLM Inference Serving

The widespread adoption of Large Language Models (LLMs) has enabled diverse applications with very different latency requirements. Existing LLM serving frameworks rely on siloed infrastructure with coarse-grained workload segregation -- interactive and batch -- leading to inefficient resource utilization and limited support for fine-grained Quality-of-Service (QoS) differentiation. This results in operational inefficiencies, over-provisioning and poor load management during traffic surges. We present Niyama, a novel QoS-driven inference serving system that enables efficient co-scheduling of diverse workloads on shared infrastructure. Niyama introduces fine-grained QoS classification allowing applications to specify precise latency requirements, and dynamically adapts scheduling decisions based on real-time system state. Leveraging the predictable execution characteristics of LLM inference, Niyama implements a dynamic chunking mechanism to improve overall throughput while maintaining strict QoS guarantees. Additionally, Niyama employs a hybrid prioritization policy that balances fairness and efficiency, and employs selective request relegation that enables graceful service degradation during overload conditions. Our evaluation demonstrates that Niyama increases serving capacity by 32% compared to current siloed deployments, while maintaining QoS guarantees. Notably, under extreme load, our system reduces SLO violations by an order of magnitude compared to current strategies.

==> figures/eval_goodput.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
         \includegraphics[width=\linewidth]{graphs/capacity.pdf}
         \caption{Capacity to serve a load of 50 QPS}
         \label{fig:eval:gpus}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.45\textwidth}
         \includegraphics[width=\linewidth]{graphs/goodput.pdf}
         \caption{Maximum goodput in a shared cluster}
         \label{fig:eval:goodput}
     \end{subfigure}
     \vspace{-1em}
        \caption{Capacity evaluation at uniform load}
        \vspace{1em}
\end{figure}


==> figures/eval_gpus.tex <==
\begin{figure}[!t]
    \centering
        \includegraphics[width=0.95\linewidth]{graphs/capacity.pdf}
        \caption{Capacity required to serve a load of 50QPS per QoS bucket across SOTA siloed infrastructure and \sysname }
    \label{fig:eval:gpus}
\end{figure}

==> sections/1-abstract-v2.tex <==
\begin{abstract}
The widespread adoption of Large Language Models (LLMs) across billions of users and diverse applications has introduced unprecedented challenges in scalable inference deployment. Current deployments rely on siloed infrastructure and lack mechanisms to express nuanced latency requirements, resulting in operational inefficiencies, over provisioning and poor load management during traffic surges.

We present \sysname, a novel QoS-driven inference serving system that addresses these limitations through two key innovations. First, we introduce fine-grained QoS bucketing that enables co-scheduling requests with diverse latency targets on shared infrastructure. By exploiting the predictable execution characteristics of LLM inference, our system dynamically adjusts chunk sizes to improve overall throughput. Second, we develop a hybrid prioritization policy with selective request dropping that enables graceful service degradation during overload conditions, balancing fairness with performance.
Our evaluation demonstrates that \sysname increases serving capacity by 32\% compared to current siloed deployments while maintaining QoS guarantees. Even under extreme load, our system reduces SLO violations by an order of magnitude compared to current strategies.

%ensures that a high percentage of requests meet their latency targets by selectively degrading service for less critical workloads. This approach represents a fundamental reimagining of LLM inference infrastructure, transforming computational resource management from static allocation to dynamic, application-aware ecosystems.
\end{abstract}

==> sections/1-abstract.tex <==
\begin{abstract}
The widespread adoption of Large Language Models (LLMs) across billions of users and diverse applications has introduced unprecedented challenges in scalable inference deployment. While prior work has focused primarily on improving performance, the tradeoff between cost efficiency and Quality of Service (QoS) in production deployments remain underexplored. We present a \sysname, a system for LLM inference serving that addresses these challenges through QoS-aware scheduling and dynamic load management. \sysname introduces  QoS classes with associated Service Level Objectives (SLOs), coupled with a novel hybrid scheduling approach that leverages application-provided hints for intelligent resource allocation. Through extensive evaluation on production workloads, we demonstrate that \sysname achieves upto 20\% higher serving throughput while maintaining strict QoS guarantees. Our overload management techniques reduce request denials and SLO violations by $10\times$ during load spikes compared to existing approaches. 
\end{abstract}

==> sections/4-design-v2.tex <==
\section{\sysname: Design and Implementation}
\sysname efficiently manages concurrent LLM inference requests with diverse QoS requirements while maximizing resource utilization across shared infrastructure. ~\cref{fig:system_design} illustrates the high-level components and interactions within our system. 

\sysname uses a two-stage pipeline to manage requests. When requests arrive from various applications, they enter replica-level queues where our \emph{hybrid prioritization policy} evaluates them based on both deadline proximity and request length. In each scheduling iteration, the policy selects the most appropriate prefill request(s) for processing.
Before assembling a new batch, \sysname's scheduler first examines all active decode requests against their target deadlines. The scheduler uses \emph{eager relegation} to temporarily move any decode requests that have already exceeded their latency constraints to a releagted queue, allowing the system to maintain responsiveness for requests that can still meet their deadlines.
The scheduler then exploits the predictability of LLM inference latency given its batch composition to dynamically construct optimized token batches by combining all remaining decode tokens with prefill tokens from newly selected requests. The \emph{dynamic chunking} mechanism carefully calculates the optimal batch size that ensures no requests in the current batch will violate their latency requirements. This mixed batch of prefill and decode tokens is then dispatched to the GPU for model execution.

\sysname thus offers a graceful degradation of service during overloads  by returning to the relegated requests during periods of lower system load. When the primary request queue is empty or system utilization drops, the scheduler begins processing these temporarily delayed requests, ensuring that all workloads eventually complete rather than being permanently rejected. This approach balances immediate responsiveness with overall throughput efficiency.

%Unlike traditional inference systems that segregate workloads into separate clusters based on broad service categories, \sysname enables fine-grained co-scheduling of requests with varying latency requirements on the same infrastructure. This approach is particularly valuable for organizations experiencing fluctuating workload patterns throughout the day, where rigid resource allocation leads to inefficient utilization. We now describe each component of \sysname in detail.

\subsection{Expanding the serving API}
Each incoming request to Niyama is characterized by multiple attributes that inform scheduling decisions: prefill length (number of tokens in the input prompt), expected decode length (estimated number of tokens to be generated), and QoS bucket. The QoS bucket defines the request's service level objective through Time To First Token (TTFT), which specifies the maximum allowable time before the first token is generated, and Time Between Tokens (TBT), which defines the maximum allowable time between consecutive token generations. Additionally, each request has an associated priority level indicating its relative importance compared to others in the system.
Following the approach in~\cite{metron}, we enforce that the first token must be delivered within TTFT, and the i-th token must be delivered within TTFT + (i-1) × TBT time units. This creates a progressive deadline schedule for each token in the sequence, allowing for precise tracking of SLO compliance throughout the request lifecycle. The QoS bucketing mechanism enables applications to express their specific requirements. For example, an interactive chat application might specify a TTFT of 200ms and a TBT of 50ms with high priority, while a document summarization service might request a TTFT of 2000ms and a TBT of 100ms with medium priority. This granular expression of requirements is critical for effective resource sharing across diverse workloads.
3.3 Scheduling Mechanism
Niyama's scheduling system optimizes for two potentially conflicting objectives: maximizing resource utilization and ensuring requests meet their QoS targets. Our approach leverages the unique execution characteristics of LLM inference to achieve both goals.
3.3.1 Decode-First Batching Strategy
A key insight driving our design is that decode operations maintain state in GPU memory through their KV-cache, making it beneficial to process them promptly and continuously. Our system implements a decode-first batching strategy to minimize memory pressure and improve resource utilization. For each processing cycle, all pending decode requests (D tokens) are included in the current batch to ensure the KV-cache of each request remains in the system for the minimal required duration. Prefill tokens are then added opportunistically to utilize remaining capacity.
This approach differs significantly from traditional FCFS batching strategies that might mix prefill and decode operations without considering their distinct resource usage patterns. By prioritizing decode operations, we ensure continuous progress on active generations while efficiently utilizing any remaining capacity for new requests.
3.3.2 Dynamic Chunk Size Selection
The total number of tokens processed in a batch (chunk size C) significantly impacts both throughput and latency. As shown in Figure 2, throughput increases with chunk size until reaching a knee point, after which latency begins to increase dramatically due to memory swapping and reduced parallelism efficiency. Niyama's scheduler dynamically determines the optimal chunk size C based on the minimum slack available among all decode requests in the current batch and offline profiling data that maps slack values to optimal chunk sizes.
This dynamic approach allows us to adapt to changing system conditions in real-time. When all requests have ample slack (time remaining before their deadlines), the system can process larger chunks to maximize throughput. As deadlines approach, the chunk size is reduced to ensure timely processing of critical requests. We implemented an offline profiling system that characterizes the relationship between chunk size, system load, and processing latency across different hardware configurations. This data is compiled into a lookup table that the scheduler consults during runtime to make informed decisions about optimal chunk sizes without requiring expensive online profiling.
3.3.3 Hybrid Prioritization Policy
Niyama implements a novel hybrid prioritization policy that creates a continuum between first-come-first-served (FCFS) and shortest-job-first (SJF) scheduling approaches. This policy addresses the inherent trade-off between fairness and efficiency. Under normal load conditions, the system tends toward FCFS to ensure fairness and prevent starvation. As system load increases, the policy gradually shifts toward SJF for critical requests, prioritizing shorter jobs that can be completed quickly.
This adaptive approach is implemented through a dynamic scoring function that assigns each request a priority score: Priority_Score = α × (Deadline_Proximity) + (1-α) × (Original_Queue_Position), where α is dynamically adjusted based on system load, ranging from 0 (pure FCFS) to 1 (pure deadline-based scheduling). This formulation allows the system to smoothly transition between scheduling regimes as conditions change, rather than making abrupt policy shifts.
3.3.4 Earliest-Deadline-First Queue Management with Selective Relegation
The prefill request queue is maintained in Earliest-Deadline-First (EDF) order based on TTFT deadlines. For each scheduling cycle, after determining the optimal chunk size C and accounting for D decode tokens, we select (C-D) prefill tokens according to a specific procedure. First, we examine the head of the prefill queue and perform an SLO feasibility check to determine if the request can meet its deadline constraints. If the deadline cannot be met, rather than processing the request immediately (which would cause head-of-line blocking), we relegate it to a secondary lower-priority queue. We continue this process until we have selected (C-D) prefill tokens or exhausted the queue.
This relegation mechanism is crucial for graceful degradation under high load conditions. By contrast, a simple FCFS approach would lead to all requests suffering from increased latency due to head-of-line blocking effects. Our approach ensures that a small percentage of requests experience significant degradation while maintaining QoS for the majority.
3.4 Intelligent Load Shedding
Beyond queue management, Niyama incorporates intelligent load shedding to maintain system stability during extreme overload conditions. Unlike simplistic throttling approaches that indiscriminately reject incoming requests, our system makes informed decisions based on current system load and projected processing capacity, the QoS bucket and priority level of each incoming request, and historical patterns of request completion success rates.
When the system determines that incoming load exceeds processing capacity, it selectively rejects or delays requests based on their priority levels and estimated resource requirements. This approach ensures that high-priority requests continue to meet their SLOs while lower-priority requests may experience increased latency or rejection. Importantly, load shedding decisions are communicated to clients through a rich feedback mechanism that provides estimated wait time for delayed requests, suggested retry intervals for rejected requests, and current system status and alternative processing options. This transparent approach enables client applications to make informed decisions about how to handle their requests during overload conditions, rather than experiencing opaque failures or unpredictable latency.
3.5 Processing and Feedback Loop
Once a batch is assembled with D decode tokens and (C-D) prefill tokens, it is sent to the LLM for processing. The results are then categorized: completed prefills are moved to the decode pool for subsequent token generation, incomplete prefills are returned to the prefill queue, and completed decodes (those reaching an EOS token) exit the system. This feedback loop ensures continuous optimization of resource utilization while maintaining strict adherence to latency constraints. The system constantly monitors the progress of each request against its deadline schedule, adjusting processing priorities as needed to maintain SLO compliance.
3.6 Implementation Details
We implemented Niyama as a standalone service that integrates with popular LLM serving frameworks including vLLM [45] and TensorRT-LLM [28]. The core scheduling logic is written in C++ for performance, with a Python API layer for integration flexibility. The system runs on standard cloud infrastructure and has been tested with a variety of LLM architectures including GPT, LLaMA, and Mistral variants ranging from 7B to 70B parameters.
Key implementation challenges included efficient queue management, dynamic profiling, and fault tolerance. We implemented lock-free concurrent queues to minimize scheduling overhead while maintaining consistent priority ordering. Our system includes a lightweight profiling mechanism that continuously updates the chunk size optimization tables based on observed performance, allowing adaptation to changing hardware conditions and model characteristics. Niyama also implements checkpoint-based recovery for long-running batch requests, ensuring that system failures do not result in complete restart of expensive prefill operations.
The modular design of Niyama allows for easy extension to support new models and hardware configurations. The scheduling policies can be customized through configuration files without requiring code changes, enabling deployment teams to fine-tune the system for their specific workload characteristics and business priorities.

==> sections/4-design-v3.tex <==
\section{\sysname: Design and Implementation}
\sysname is designed to efficiently manage concurrent LLM inference requests with diverse QoS requirements, while maximizing resource utilization across the shared infrastructure. We address the limitations outlined earlier by dynamically adapting scheduling decisions based on real-time system state and QoS targets of the in flight requests. %~\cref{fig:system_design} illustrates the high-level components and interactions within our system. 

\input{figures/system-design}

\subsection{Overview}
The architecture of \sysname is shown in ~\cref{fig:system_design}. \sysname uses a two-stage pipeline to manage requests. When requests arrive from various applications, they enter replica-level queues where our \emph{hybrid prioritization policy} evaluates them based on both deadline proximity and request length. In each scheduling iteration, the policy selects the most appropriate prefill request(s) for processing.
Before assembling a new batch, \sysname's scheduler first examines if the ongoing or newly chosen prefill request has violated its deadline (or will in the current iteration). If so, the scheduler uses \emph{eager relegation} to temporarily move that request to a relegated queue, allowing the system to maintain responsiveness for requests that can still meet their deadlines.
The scheduler then exploits the predictability of LLM inference latency given its batch composition to dynamically construct optimized token batches by combining all remaining decode tokens with prefill tokens from newly selected requests. The \emph{dynamic chunking} mechanism uses a lightweight predictor to find the optimal batch size that ensures no requests in the current batch will violate their latency requirements. This mixed batch of prefill and decode tokens is then dispatched to the GPU for model execution.

When the primary request queue is empty or system utilization drops, the scheduler begins processing the relegated requests, ensuring that all workloads eventually complete rather than being permanently rejected. This approach balances immediate responsiveness with overall throughput efficiency, thus offering graceful service degradation during overloads.

We now discuss each design point in detail.

\subsection{Defining SLO buckets and deadlines}
\sysname categorizes incoming requests into two broad QoS classes based on application-defined performance requirements. First, the interactive user-facing QoS class uses two SLOs to define QoS targets; TTFT and TBT latency. This addresses both initial response time and consistent generation pacing. Second, the non-interactive QoS class uses a single TTLT SLO, focusing on overall completion time rather than incremental progress. Each application owner can instantiate one of these two QoS classes to create their own QoS bucket, allowing for customized performance guarantees tailored to specific application needs as shown in ~\cref{fig:qos-buckets}.

The deadline for each request is calculated differently based on its QoS class. For interactive QoS class, the first token deadline is set as:
\begin{equation}
    D_{first} = t_{arrival} + SLO_{TTFT}
\end{equation}

Subsequent token deadlines are calculated as:
\begin{equation}
    D_n = t_{arrival} + SLO_{TTFT} + (n - 1) \cdot SLO_{TBT}
\end{equation}
where n is the token position. This ensures consistent pacing throughout generation.

Non-interactive requests use a simpler deadline model:
\begin{equation}
    D_{total} = t_{arrival} + SLO_{TTLT}
\end{equation}

\subsection{Scheduling strategy}
After defining the deadline for each request, we need to efficiently schedule them to minimize deadline violations while maximizing throughput. Scheduling requests of different QoS classes with different latency SLOs on a shared cluster is challenging. LLM inference scheduling involves a fundamental trade-off between throughput and latency~\cite{agrawal2024taming}, i.e.,  reducing latency requires splitting user input into smaller chunks but this results in lower throughput\footnote{An alternative approach is using a disaggregated architecture~\cite{patel2023splitwise,distserve2024} but that comes with its own trade-offs.}. State-of-the-art LLM inference serving frameworks~\cite{vllm} serve requests using chunked-prefills, where every iteration process a fixed number of tokens (called chunk size), which includes both prefill and decode tokens from different requests using fused prefill-decode MLP to improve the compute efficiency of memory-bound decode phase~\cite{sarathi2023}. A larger chunk results in better throughput but also increases the TBT of the decodes in the batch as shown in ~\cref{fig:chunk-perf}. Therefore, 
interactive jobs use smaller chunk sizes (served at higher cost per token due to lower throughput) while batch jobs use larger chunk sizes (served at lower cost thanks to higher throughput).

\input{figures/chunking-tput}
\input{figures/dynamic_chunk}
\jheading{Dynamic chunking}
A naive approach to co-schedule jobs of different QoS classes with various deadlines on TTFT, TBT, and TTLT would be to use the smallest chunk size necessary to meet the latency constraint of the strictest QoS class. However, this would result in low throughput and high cost for all service
classes. 

\sysname opportunistically increases chunk size in every iteration based on the accumulated slack(time remaining before their respective deadlines) of all the requests in the current batch. Our system dynamically adjusts chunk size based on accumulated slack (time before deadlines) of all requests in the current batch. This adaptive approach responds to real-time conditions: when requests have sufficient slack, larger chunks maximize throughput; as deadlines approach, chunk sizes decrease to ensure timely processing. We leverage the predictability of LLM inference latency given its batch composition by building a lightweight predictor using offline profiles from an LLM simulator~\cite{vidur}. Building a chunk size predictor for a model-hardware combination requires only about an hour of profiling on a single target GPU. 

\Cref{fig:dynamic_chunk} illustrates our approach with five requests (A--E) across three QoS buckets, where C is interactive while others are non-interactive. State-of-the-art LLM schedulers like vllm~\cite{vllmsosp} and sarathi~\cite{sarathi2023} execute each iteration using a fixed chunk size and process requests in arrival order (FCFS). Our solution introduces two key improvements.

First, we prioritize requests based on their QoS targets using Earliest Deadline First (EDF) scheduling, which processes request C before B due to its earlier deadline. \sref{sec:sched_optimizations} details how we further adapt this traditional policy to address challenges and opportunities unique to LLM inference. Second, we dynamically adjust chunk sizes based on accumulated slack. For example, after B's prefill phase completes earlier than its deadline, it accumulates significant slack before its next token is due. We exploit this slack by dynamically increasing the chunk size, adding more prefill tokens from requests B and E (which have the earliest deadlines in the queue), thereby improving throughput without violating any ongoing request deadlines.

When the interactive job C enters its decode phase, we revert to the original smaller chunk size necessary to meet its TBT requirement, though we still exploit any slack accumulated if decoding completes faster than predicted. Once C completes and no remaining requests impose strict TBT constraints, we again increase chunk size to maximize throughput while respecting the TTLT deadlines of ongoing requests. This approach effectively leverages the predictable execution characteristics of LLMs to dynamically optimize chunk sizes during runtime, balancing throughput and deadline requirements.


\subsection{Scheduling optimizations}
\label{sec:sched_optimizations}
While dynamic chunking helps maximize throughput while meeting the requests' deadlines, naively prioritizing jobs in the request queue using traditional task scheduling with straightforward approaches like Earliest Deadline First (EDF) is suboptimal for LLM inference scheduling as it  poses unique challenges and opportunities due to its computational nature and workload characteristics: (1) the prohibitive cost of preemption during the autoregressive decode phase, where KV cache management becomes extremely expensive; (2) the complexities of overload management where standard policies like EDF can trigger cascading deadline violations while alternatives like SJF raise fairness concerns by disproportionately delaying longer requests, especially when it is tricky to define the length of a LLM request with inherently unknown decode tokens
(3) the need to handle diverse application-specific priorities across tenants in production deployments to gracefully degrade service during overloads. We now explain each of these challenges and how \sysname tackles them.

\jheading{Challenge 1 : Minimizing Preemption Costs}
Scheduling requests to minimize deadline violations requires us to enable preemptions to prevent priority inversions; i.e., a near-deadline task might be blocked by a far-deadline task. Preemption should be carefully handled in the context of LLM inference, which has two phases - prefill, a parallel, compute efficient phase with highly predictable latency and decodes, an autoregressive, memory bound phase of unknown length with low predictability. Preempting a request during the decode phase requires either migrating large KV caches in and out of GPU memory or expensive recomputation. These operations are particularly costly given tight TBT SLOs (order of a few tens of milliseconds) compared to TTFT metrics (order of a few seconds).

\sysname addresses this challenge by introducing \textbf{selective preemption}. 
\sysname preempts a request to accommodate another one with a shorter deadline only if (1) the ongoing request is in its prefill phase and (2) preempting that request for an iteration does not result in its deadline violation. In each scheduling iteration, all pending decode requests are scheduled in a batch and prefill tokens are added opportunistically to utilize any remaining capacity as done in state-of-the-art LLM scheduling~\cite{sarathi2023}. This approach ensures that the KV cache for each request remains in the GPU for the shortest necessary duration, thereby minimizing memory pressure.

\jheading{Challenge 2: Fair Overload Management}
Simple scheduling approaches for handling overloads, such as shortest job first (SJF), delay all longer requests disproportionately, resulting in fairness concerns. Although SJF can better
manage overload than EDF due to the quadratic dependence
of prompt length on LLM system load by virtue of attention computation, it implicitly prioritizes shorter requests and neglects the QoS requirements of
longer ones. 

To address this, QoServe introduces a \textbf{hybrid prioritization
policy} that smoothly interpolates between EDF and SJF,
allowing deployments to strike a balance between fairness
and efficiency. The priority of a request in the interactive QoS class is given by a linear combination of TTFT deadline and the time taken to process the remaining prefills in the request
\begin{equation}
    P_i = t_{arrival}^i + SLO_{TTFT}^i + \alpha * Prefill_{rem}^i
\end{equation}

For the interactive jobs, we only consider TTFT deadline while scheduling them; dynamic chunking takes care of meeting the corresponding TBT deadlines as we do not allow decode preemptions.

For the non-interactive QoS class, request priority is given by 
\begin{equation}
    P_i = t_{arrival}^i + SLO_{TTLT}^i + \alpha * Tokens_{rem}^i
\end{equation}
where $Tokens_{rem}$ indicate the total pending tokens (prefill + decode). Since decode length is unknown in LLM inference, this introduces a challenge in modeling the priority of non-interactive requests. We tackle this challenge using a simple insight; for non-interactive jobs, the TTLT deadline is typically much greater than their actual processing time. Therefore, given an application, we can use historic information on the decode tokens generated by that application and over-approximate it by two standard deviations. We show in \sref{sec:eval} that this simple prediction sufficiently captures the priority of non-interactive jobs.

\jheading{Challenge 3: Multi-Tenant Priority Management}
Production LLM deployments serve requests with drastically different importance levels (e.g., free-tier vs. premium users). Standard deadline-based policies fail to incorporate these application-specific priorities, missing opportunities to maintain service quality for high-value requests during resource constraints.

\sysname employs \textbf{eager relegation} to proactively degrade service for a small
subset of requests using application hints to ensure stable performance for the majority, even under extreme load conditions. The key idea is very simple; if a request has already violated its TTFT or TTLT deadline or is about to violate it in the current iteration, then \sysname de-prioritizes it into a relegated queue. In multi-tenant deployments, we use application hints such as free vs paid tier to preferentially relegate low priority requests to ensure stability of service to the high priority ones. When there are no more low priority requests, \sysname proactively relegates requests that have violated their deadlines to prevent cascading deadline violations. This enables graceful degradation of service even under extreme load. 



\subsection{Implementation}

We implemented \sysname by extending the Sarathi scheduler~\cite{sarathi2023}, which is built on top of the vLLM inference system~\cite{vllmsosp}. The implementation focuses on enhancing the scheduler component while maintaining compatibility with vLLM's efficient tensor parallelism and PagedAttention mechanisms. We extended the vLLM API to associate each inference request with its corresponding QoS requirements (TTFT, TBT, and/or TTLT) and priority level during request submission. The dynamic chunk size predictor is implemented as a lightweight random forest model trained on performance profiles collected from the Vidur LLM inference simulator~\cite{vidur}, adding minimal overhead to the scheduling process. The hybrid prioritization policy is implemented using a priority queue that incorporates both deadline proximity and estimated processing time, with the interpolation factor $\alpha$ configurable as a deployment parameter. For non-interactive requests, we maintain a running history of token generation patterns per application to estimate the expected decode length. The eager relegation mechanism tracks the running throughput of the system, estimates the expected processing time of each request, and determines whether to relegate a request based on these metrics. Relegated requests remain within the same scheduler, residing in a lower-priority queue that may be serviced during periods of lower system load. To support multi-tenant deployments, we added a priority field to each request that enables informed relegation decisions based on application hints such as free-tier versus premium users.

==> sections/4-design.tex <==
\section{Design and Implementation of \sysname}

\input{figures/system-design}

\subsection{Overview}
Our LLM serving system architecture is designed to efficiently manage concurrent inference requests while maintaining strict latency requirements. Figure~\ref{fig:system_design} illustrates the high-level components and interactions within our system.

\subsection{Request Processing Model}
Each incoming request to our system is characterized by its prefill length, expected decode length, and latency constraints. These constraints are expressed as:
\begin{itemize}
    \item \textbf{Time To First Token (TTFT)}: Maximum allowable time before the first token is generated
    \item \textbf{Time Between Tokens (TBT)}: Maximum allowable time between consecutive token generations
    \item \textbf{Time To Last Token (TTLT)}: Maximum allowable time before the last token is generated.
\end{itemize}

For Interactive jobs with TTFT and TBT constraints, following the approach in \citet{etalon2024}, we enforce that the first token must be delivered within TTFT, and the $i$-th token must be delivered within $\text{TTFT} + (i-1) \times \text{TBT}$ time units. This creates a progressive deadline schedule for each token in the sequence. For TTLT constraints, we design a similar schedule to above by approximating the number of output tokens.

\begin{align}
\text{TTLT} &= \text{TTFT} + (\text{num\_output\_tokens} - 1) \cdot \text{TBT} \\
\text{TTFT} &= \text{TTLT} - (\text{num\_output\_tokens} - 1) \cdot \text{TBT}
\end{align}

This equation is used to estimate the Time To First Token (TTFT) when the Time To Last Token (TTLT) constraint is provided. By rearranging the formula, we can calculate the maximum allowable TTFT to ensure the TTLT constraint is satisfied, accounting for the time needed to generate all tokens after the first one. Here prior works on output length prediction  \cite{qiu2024efficientinteractivellmserving} \cite{zheng2023responselengthperceptionsequence} is useful, however we find that overestimating the output tokens doesn't lead to significant throughput loss, hence we use the maximum output length as the prediction. This conservative approach ensures that all latency constraints are satisfied, even when the actual output length varies from the prediction.

\subsection{Scheduling Mechanism}

\subsubsection{Decode-First Batching Strategy}
Our system implements a decode-first batching strategy to minimize memory pressure and improve resource utilization. For each processing cycle:

\begin{enumerate}
    \item All pending decode requests ($D$ tokens) are included in the current batch to ensure the KV-cache of each request remains in the system for the minimal required duration.
    \item Prefill tokens are then added opportunistically to utilize remaining capacity.
\end{enumerate}

This approach is motivated by the observation that decode operations maintain state in GPU memory through their KV-cache, making it beneficial to process them promptly and continuously.

\subsubsection{Dynamic Chunk Size Selection}
The total number of tokens processed in a batch (chunk size $C$) significantly impacts both throughput and latency. As shown in Figure~\ref{fig:chunk-perf}, throughput increases with chunk size until reaching a knee point, after which latency begins to increase dramatically.



Our scheduler dynamically determines the optimal chunk size $C$ based on:
\begin{enumerate}
    \item The minimum slack available among all decode requests in the current batch
    \item Offline profiling data that maps slack values to optimal chunk sizes
\end{enumerate}

This approach allows us to maximize throughput while ensuring that all deadline constraints are satisfied.

\subsubsection{Earliest-Deadline-First Queue Management}
The prefill request queue is maintained in Earliest-Deadline-First (EDF) order based on TTFT deadlines. For each scheduling cycle, after determining the optimal chunk size $C$ and accounting for $D$ decode tokens, we select $(C-D)$ prefill tokens according to the following procedure:

\begin{enumerate}
    \item Examine the head of the prefill queue.
    \item Perform an SLO feasibility check to determine if the request can meet its deadline constraints.
    \item If the deadline cannot be met, we make a critical design decision: rather than processing the request immediately (which would cause head-of-line blocking), we relegate it to a secondary lower-priority queue.
    \item Continue this process until we have selected $(C-D)$ prefill tokens or exhausted the queue.
\end{enumerate}

This relegation mechanism is crucial for graceful degradation under high load conditions, as demonstrated in our evaluation (Section~\ref{sec:evaluation}). By contrast, a simple First-Come-First-Served approach would lead to all requests suffering from increased latency due to head-of-line blocking effects.

\subsection{Processing and Feedback Loop}
Once a batch is assembled with $D$ decode tokens and $(C-D)$ prefill tokens, it is sent to the LLM for processing. The results are then categorized:

\begin{itemize}
    \item Completed prefills are moved to the decode pool for subsequent token generation
    \item Incomplete prefills are returned to the prefill queue
    \item Completed decodes (those reaching an EOS token) exit the system
\end{itemize}

This feedback loop ensures continuous optimization of resource utilization while maintaining strict adherence to latency constraints.

==> tables/results_code.tex <==
% Place this in sections/5-eval.tex where you want the table to appear


\begin{table*}[t]
\caption{Comparison of different scheduling policies and their performance metrics}
\label{tab:scheduling-policies}
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r}
\toprule
\textbf{Policy} & \textbf{QPS} & \textbf{Tier 0} & \textbf{Tier 1} & \textbf{Tier 2} & \textbf{Batch} & \textbf{Prefill} & \textbf{Decode} & \textbf{1280} & \textbf{768} & \textbf{256} & \textbf{Other} \\
& & \textbf{(6s)} & \textbf{(600s)} & \textbf{(1800s)} & \textbf{Count} & \textbf{Only} & \textbf{Only} & \textbf{Chunk} & \textbf{Chunk} & \textbf{Chunk} & \textbf{Chunk} \\
\midrule
nFCFS(42K) & 2.6 & 0.72 & 0.00 & 0.00 & 666,291 & 227 & 326,300 & 135 & 0 & 323,900 & 342,256 \\
nFCFS(42K) & 3.0 & 5.37 & 0.00 & 0.00 & 507,659 & 97 & 167,109 & 54 & 0 & 331,050 & 176,555 \\
nFCFS(42K) & 3.4 & 65.95 & 0.00 & 0.00 & 366,398 & 54 & 25,105 & 31 & 0 & 339,853 & 26,514 \\
\addlinespace[0.5em]
nFCFS+DC(42K) & 3.0 & 0.75 & 0.00 & 0.00 & 473,760 & 87 & 388,243 & 50,310 & 1,039 & 7,094 & 415,317 \\
nFCFS+DC(42K) & 3.4 & 7.44 & 0.00 & 0.00 & 339,829 & 67 & 218,627 & 42,210 & 7,163 & 53,149 & 237,307 \\
nFCFS+DC(42K) & 3.8 & 100.00 & 0.00 & 0.00 & 272,415 & 60 & 9,547 & 919 & 37,194 & 224,399 & 9,903 \\
\addlinespace[0.5em]
EDF(112K) & 3.4 & 0.09 & 0.00 & 0.00 & 895,969 & 16 & 78,965 & 8 & 0 & 811,630 & 84,331 \\
EDF(292K) & 3.8 & 91.94 & 92.71 & 94.39 & 2,041,187 & 1 & 625 & 1 & 0 & 2,040,560 & 626 \\
\addlinespace[0.5em]
dEDF(112K) & 3.4 & 0.06 & 0.00 & 0.00 & 890,659 & 28 & 73,668 & 15 & 0 & 812,101 & 78,543 \\
dEDF(292K) & 3.8 & 2.97 & 2.86 & 2.91 & 2,041,297 & 2 & 735 & 2 & 0 & 2,040,559 & 736 \\
dEDF(172K) & 4.2 & 6.32 & 6.33 & 6.07 & 1,225,647 & 3 & 882 & 3 & 0 & 1,224,761 & 883 \\
\addlinespace[0.5em]
dEDF+DC(112K) & 3.4 & 0.05 & 0.00 & 0.00 & 811,514 & 35 & 567,584 & 114,529 & 8,070 & 71,476 & 617,439 \\
dEDF+DC(292K) & 3.8 & 0.26 & 0.00 & 0.00 & 1,441,861 & 4 & 479,306 & 207,643 & 72,232 & 631,201 & 530,785 \\
dEDF+DC(322K) & 4.2 & 3.27 & 3.30 & 3.20 & 1,561,612 & 638 & 2 & 76,044 & 189,801 & 1,295,128 & 639 \\
dEDF+DC(337K) & 4.4 & 6.00 & 5.86 & 5.81 & 1,744,379 & 772 & 2 & 42,863 & 215,439 & 1,485,304 & 773 \\
\addlinespace[0.5em]
dEDF+DC+C(322K) & 4.2 & 2.35 & 2.17 & 2.20 & 1,506,679 & 617 & 1 & 106,180 & 156,987 & 1,242,894 & 618 \\
dEDF+DC+C(337K) & 4.4 & 3.86 & 3.76 & 3.66 & 1,648,234 & 704 & 1 & 85,446 & 178,313 & 1,383,770 & 705 \\
\bottomrule
\end{tabular}
\end{table*}

